Optimal Voltage Phasor Regulation for Switching Actions in Unbalanced Distribution Systems

The proliferation of phasor measurement units (PMUs) into electric power distribution grids presents new opportunities for utility operators to manage distribution systems more effectively. One potential application of PMU measurements is to facilitate distribution grid re-configuration. Given the increasing amount of Distributed Energy Resource (DER) penetration into distribution grids, in this work we formulate an Optimal Power Flow (OPF) approach that manages DER power injections to minimize the voltage phasor difference between two nodes on a distribution network to enable efficient network reconfiguration. In order to accomplish this, we develop a linear model that relates voltage phase angles to real and reactive power flows in unbalanced distribution systems. Used in conjunction with existing linearizations relating voltage magnitude differences to power flows, we formulate an OPF capable of minimizing voltage phasor differences across different points in the network. In simulations, we explore the use of the developed approach to minimize the phasor difference across switches to be opened or closed, thereby providing an opportunity to automate and increase the speed of reconfigurations in unbalanced distribution grids.

==> responseletter.tex <==
Dear Editor and Reviewers,

We wish to express our gratitude for your reviews and invaluable feedback. We appreciate your time and effort in reviewing our submission and have made several changes to our work to reflect your feedback and comments.

% Editor

In Section 4, we added a second experiment on a larger network with multiple switching actions to demonstrate the advantages of the OPF formulation. We also discuss the advantages of the linearized model and its incorporation into an OPF, as well the disadvantages and possible ways to overcome them.

In Section 4B, we expanded our first experiment to include Volt-VAr control (VVC). We incorporated a VVC model into the OPF, to capture the effect of uncontrolled devices performing voltage regulation.

% Reviewer 1

We have clarified the explanation of our methods and results for the model accuracy analysis in Section 3.

In Section 2, we have rewritten portions of the model derivation to clarify the linearizing assumptions .

% Review 2

1 - In Section 4D, how the OPF can be modified to include multiple networks connected to the same transmission line, or multiple disconnected networks.

2 - In Section 4C, we perform a simulation on a network with two sequential switching actions. We solve the OPF for each switching action, and provide power flow results for each switch closing.

3 - 

4 - In Section 4D, we discuss of the limitations of the power flow model, in the context of the results of Section 3. We also briefly discuss how to overcome these limitations.

% Reviewer 3

1 - What the hell do they mean?

2 - In Section 4A, we discuss our previous efforts in formulating semidefinite relaxation OPFs, incorporating the angle equation of (25) or (26), with similar objectives as the OPF in our work. We discuss the success and failures of our simulations, which motivating our present work.

3 - We added a brief note on expanding the power flow model for nodes with a transformer between them, using the analysis in ``Distribution System Modeling and Analysis'' by Kersting.

4 - We did not do

5 - In Section 4B and 4C We provide discussion of our choice of the OPF objective function weightings

6 - In Section 4A and 4B, we provide discussion of why we consider four-quadrant DER operation, as we want to consider future DER operations such as battery charging.

7 - In Section 4A, we clarify that the OPF we propose is not economically motivated, and that economic activity would be suspended in favor of grid reconfiguration operations.

Sincerely,

==> temp.tex <==
\path (inf) ++(-7,-3) node[draw, ultra thick, inner sep=2pt] (2799) {\LARGE 2799};
\draw[ultra thick] (inf) -- ++(0,-1.5) -| (2799);

\path (2799) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2701) {\LARGE 2701};
\draw[ultra thick] (2799) -- (2701);

\path (2701) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2702) {\LARGE 2702};
\draw[ultra thick] (2701) -- (2702);

\path (2702) ++(-2,0) node[draw, ultra thick, inner sep=2pt] (2705) {\LARGE 2705};
\draw[ultra thick] (2702) -- (2705);

\path (2705) ++(0,1.75) node[draw, ultra thick, inner sep=2pt] (2712) {\LARGE 2712};
\draw[ultra thick] (2705) -- (2712);

\path (2705) ++(-2,0) node[draw, ultra thick, inner sep=2pt] (2742) {\LARGE 2742};
\draw[ultra thick] (2705) -- (2742);

\path (2702) ++(2,0) node[draw, ultra thick, inner sep=2pt] (2713) {\LARGE 2713};
\draw[ultra thick] (2702) -- (2713);

\path (2713) ++(2,0) node[draw, ultra thick, inner sep=2pt] (2704) {\LARGE 2704};
\draw[ultra thick] (2713) -- (2704);

\path (2704) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2714) {\LARGE 2714};
\draw[ultra thick] (2704) -- (2714);

\path (2714) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2718) {\LARGE 2718};
\draw[ultra thick] (2714) -- (2718);

\path (2704) ++(2,0) node[draw, ultra thick, inner sep=2pt] (2720) {\LARGE 2720};
\draw[ultra thick] (2704) -- (2720);

\path (2720) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2706) {\LARGE 2706};
\draw[ultra thick] (2720) -- (2706);

\path (2706) ++(0,-1.75) node[draw, ultra thick, inner sep=3pt] (2725) {\LARGE 2725};
\draw[ultra thick] (2706) -- (2725);

\path (2720) ++(0,1.75) node[draw, ultra thick, inner sep=2pt] (2707) {\LARGE 2707};
\draw[ultra thick] (2720) -- (2707);

\path (2707) ++(0,1.75) node[draw, ultra thick, inner sep=2pt] (2724) {\LARGE 2724};
\draw[ultra thick] (2707) -- (2724);

\path (2707) ++(-2,0) node[draw, ultra thick, inner sep=2pt] (2722) {\LARGE 2722};
\draw[ultra thick] (2707) -- (2722);

\path (2702) ++(0,-3.5) node[draw, ultra thick, inner sep=2pt] (2703) {\LARGE 2703};
\draw[ultra thick] (2702) -- (2703);

\path (2703) ++(-2,0) node[draw, ultra thick, inner sep=2pt] (2727) {\LARGE 2727};
\draw[ultra thick] (2703) -- (2727);

\path (2727) ++(-2,0) node[draw, ultra thick, inner sep=2pt] (2744) {\LARGE 2744};
\draw[ultra thick] (2727) -- (2744);

\path (2744) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2728) {\LARGE 2728};
\draw[ultra thick] (2744) -- (2728);

\path (2744) ++(0,1.75) node[draw, ultra thick, inner sep=2pt] (2729) {\LARGE 2729};
\draw[ultra thick] (2744) -- (2729);

\path (2703) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2730) {\LARGE 2730};
\draw[ultra thick] (2703) -- (2730);

\path (2730) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2709) {\LARGE 2709};
\draw[ultra thick] (2730) -- (2709);

\path (2709) ++(2,0) node[draw, ultra thick, inner sep=2pt] (2731) {\LARGE 2731};
\draw[ultra thick] (2709) -- (2731);

\path (2709) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2775) {\LARGE 2775};
\draw[ultra thick] (2709) -- (2775);

\path (2709) ++(-2,0) node[draw, ultra thick, inner sep=2pt] (2708) {\LARGE 2708};
\draw[ultra thick] (2709) -- (2708);

\path (2708) ++(-2,0) node[draw, ultra thick, inner sep=2pt] (2732) {\LARGE 2732};
\draw[ultra thick] (2708) -- (2732);

\path (2708) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2733) {\LARGE 2733};
\draw[ultra thick] (2708) -- (2733);

\path (2733) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2734) {\LARGE 2734};
\draw[ultra thick] (2733) -- (2734);

\path (2734) ++(-2,0) node[draw, ultra thick, inner sep=2pt] (2710) {\LARGE 2710};
\draw[ultra thick] (2734) -- (2710);

\path (2710) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2735) {\LARGE 2735};
\draw[ultra thick] (2710) -- (2735);

\path (2710) ++(0,1.75) node[draw, ultra thick, inner sep=2pt] (2736) {\LARGE 2736};
\draw[ultra thick] (2710) -- (2736);

\path (2734) ++(0,-1.75) node[draw, ultra thick, inner sep=2pt] (2737) {\LARGE 2737};
\draw[ultra thick] (2734) -- (2737);

\path (2737) ++(2,0) node[draw, ultra thick, inner sep=2pt] (2738) {\LARGE 2738};
\draw[ultra thick] (2737) -- (2738);

\path (2738) ++(2,0) node[draw, ultra thick, inner sep=2pt] (2711) {\LARGE 2711};
\draw[ultra thick] (2738) -- (2711);

\path (2711) ++(2,0) node[draw, ultra thick, inner sep=2pt] (2741) {\LARGE 2741};
\draw[ultra thick] (2711) -- (2741);

\path (2711) ++(0,1.75) node[draw, ultra thick, inner sep=2pt] (2740) {\LARGE 2740};
\draw[ultra thick] (2711) -- (2740);
